How to Elect a Leader Faster than a Tournament

The problem of electing a leader from among $n$ contenders is one of the fundamental questions in distributed computing. In its simplest formulation, the task is as follows: given $n$ processors, all participants must eventually return a win or lose indication, such that a single contender may win. Despite a considerable amount of work on leader election, the following question is still open: can we elect a leader in an asynchronous fault-prone system faster than just running a $\Theta(\log n)$-time tournament, against a strong adaptive adversary? In this paper, we answer this question in the affirmative, improving on a decades-old upper bound. We introduce two new algorithmic ideas to reduce the time complexity of electing a leader to $O(\log^* n)$, using $O(n^2)$ point-to-point messages. A non-trivial application of our algorithm is a new upper bound for the tight renaming problem, assigning $n$ items to the $n$ participants in expected $O(\log^2 n)$ time and $O(n^2)$ messages. We complement our results with lower bound of $\Omega(n^2)$ messages for solving these two problems, closing the question of their message complexity.

==> renameanalysis.tex <==
%!TEX root = main.tex
We begin by showing the correctness of the algorithm, proof of which can be 
        found in~\appendixref{app:renproofs}.
\begin{replemma}{lem:renameterminate}
The renaming algorithm in~\figureref{fig:rename} ensures termination in the presence of at most 
        $\lceil n/2 \rceil -1$ processor faults
        and no two processors return the same name from the \lit{getName} call.
\end{replemma}
\noindent We then focus on message complexity.
We begin by introducing some notation. 
For an arbitrary execution, and for every name $u$, consider the first time when more than 
        half of processors have $\id{Contended}[u] = \lit{true}$ in their view
        (or time $\infty$, if this never happens).
Let $\prec$ denote the name ordering based on these times, and 
        let $\{u_i\}$ be the sequence of names sorted according to increasing $\prec$.
Among the names with time $\infty$, sort later the ones that are never contended by the processors.
Resolve all the remaining ties according to the order of the names.
This ordering has the following useful temporal property.
\begin{lemma}
\label{lem:renameorder}
In any execution, if a processor views $\id{Contended}[i] = \lit{true}$ 
        in some while loop iteration, 
        and then, in some subsequent iteration at line~\ref{line:pickspot} the same 
        processor views $\id{Contended}[j] = \lit{false}$, $i \prec j$ has to hold.
\end{lemma}
\begin{proof}
Clearly, $j \neq i$ because contention information never disappears
        from a processor's view.
In the earlier iteration, the processor propagates 
        $\id{Contended}[i]=\lit{true}$ to more than half of the processors
        at line~\ref{line:prepropcontend} or~\ref{line:propcontend}.
During the subsequent iteration, at line~\ref{line:colContended},
        the processor collects information and does not set 
        $\id{Contended}[j]$ to $\lit{true}$ before reaching line~\ref{line:pickspot}.
Thus, more than half of the processors view
        $\id{Contended}[j] = \lit{false}$ at some intermediate time point.
Therefore, a quorum of processors views $\id{Contended}[i]=\lit{true}$
        strictly earlier than $\id{Contended}[j]=\lit{true}$, 
        and by definition $i \prec j$ has to hold.
\end{proof}
\noindent Let $X_i$ be a random variable, denoting the number of processors 
        that ever contend in a Test-and-Set for the name $u_i$. 
The following holds.
\begin{replemma}{lem:msgrenameweak}
The message complexity of our renaming algorithm is
        $O(n \cdot \mathbb{E}[\sum_{i=1}^n X_i])$. 
\end{replemma}
\noindent 
Let us partition names $\{u_i\}$ into $\log{n}$ \emph{groups}, 
        where the first group $G_1$ contains the first $n/2$ names, 
        the second group $G_2$ contains the next $n/4$ names, etc.
We will use notations $G_{j' \geq j}$, $G_{j'' > j}$ and $G_{j''' < j}$ to denote 
        the union of all groups $G_{j'}$ where $j' \geq j$, 
        all groups $G_{j''}$ where $j'' > j$,
        and all groups $G_{j'''}$ where $j''' < j$, respectively.
We can now split any execution into at most $\log{n}$ phases.
The first phase starts when the execution starts and ends as soon as for each $u_i \in G_1$ 
        more than half of the processors view $\id{Contended}[u_i] = \lit{true}$ 
        (the way $\{u\}$ is sorted, this is the same as when 
        the contention information about $u_{n/2}$ is propagated to a quorum). 
At this time, the second phase starts and ends when for each $u_i \in G_2$
        more than half of the processors view $\id{Contended}[u_i] = \lit{true}$.
When the second phase ends, the third phase starts, and so on.

Consider any loop iteration of some processor $p$ in some execution.
We say that an iteration \emph{starts} at a time instant when $p$ executes line~\ref{line:while} 
        and reaches line~\ref{line:colContended}.
Let $V_p$ be $p$'s view of the $\id{Contended}$ array
        right before picking a spot at line~\ref{line:pickspot} in the given iteration:
\vspace{3pt}
\begin{adjustwidth}{1cm}{1cm}
We say that an iteration is $\id{clean}(j)$,
        if the iteration starts during phase $j$
        and no name from later groups $G_{j'' > j}$ is contended in $V_p$.       
\vspace{2pt}
        
\noindent We say that an iteration is $\id{dirty}(j)$,
        if the iteration starts during phase $j$
        and some name from a later group $G_{j'' > j}$ is contended in $V_p$.
\end{adjustwidth}
\vspace{3pt}
\noindent Observe that any iteration that starts in phase $j$ can be uniquely classified as 
        $\id{clean}(j)$ or $\id{dirty}(j)$ and in these iterations,
        processors view all names $u_i \in G_{j''' < j}$ from previous groups as contended.
\begin{lemma}
\label{lem:ncontend}
In any execution, at most $\frac{n}{2^{j-1}}$ processors ever contend for names 
        from groups $G_{j' \geq j}$.
\end{lemma}
\begin{proof}
If no name from $G_{j' \geq j}$ is ever contended, then the statement is 
        trivially true.
On the other hand, if some name from $G_{j' \geq j}$ is ever contended, 
        then by our ordering so are all names from the former groups.
(Otherwise, an uncontended name from earlier groups would have time $\infty$ 
        and the least priority and would be sorted later).
There are $n-\frac{n}{2^{j-1}}$ names in earlier groups.
Since they all are contended at some time, there are $n-\frac{n}{2^{j-1}}$
        processors that can be linearized to win the corresponding 
        \lit{AdaptiveTAS} protocols and the name.
Consider one of these processors $p$ and the name $u$ from some earlier group
        $G_{j''' < j}$, that $p$ is bound to win.
Processor $p$ will not contend for names after $u$, and it also 
        never contended for a name from $G_{j' \geq j}$ before contending 
        for $u$, because that would have violated~\lemmaref{lem:renameorder}.
Thus, none of the $n-\frac{n}{2^{j-1}}$ processors ever contend for a
        name from $G_{j' \geq j}$, out of $n$ processors in total, 
        completing the argument. 
\end{proof}
\begin{lemma}
\label{lem:phaseunion}
For any fixed $j$, the total number of $\id{clean}(j)$ iterations
        is larger than or equal to $\alpha n + \frac{n}{2^{j-1}}$ with probability 
        at most $e^{-\frac{\alpha n}{16}}$ for all $\alpha \geq \frac{1}{2^{j-5}}$.
\end{lemma}
\begin{proof}
Fix some $j$.
Consider a time $t$ when the first $\id{dirty}(j)$ iteration is completed.
At this time, there exists an $i$ such that $u_i \in G_{j''>j}$ and more than half 
        of the processors view $\id{Contended}[i] = \lit{true}$, so all iterations 
        that start later will set $\id{Contended}[i] \gets \lit{true}$ at line~\ref{line:setcont}.
Therefore, any iteration that starts after time $t$ will observe $\id{Contended}[i] = \lit{true}$ 
        at line~\ref{line:pickspot} and by definition cannot be $\id{clean}(j)$.
By~\lemmaref{lem:ncontend}, at most $\frac{n}{2^{j-1}}$ processors
        can have active $\id{clean}(j)$ iterations at time $t$.
The total number of $\id{clean}(j)$ iterations is thus upper bounded by 
        $\frac{n}{2^{j-1}}$ plus the number of $\id{clean}(j)$ 
        iterations completed before time $t$, which we denote as \emph{safe} iterations.\footnote{
If no $\id{dirty(j)}$ iteration ever completes, then we call all $\id{clean(j)}$ iterations safe.
}

Let us now consider only safe iterations that, by definition, all finish before 
        any iteration where a processor contends for a name in $G_{j''>j}$ is completed.
%Therefore, no processor contends for a name in $G_{j''>j}$ twice.
By~\lemmaref{lem:ncontend}, at most $\frac{n}{2^{j}}$ different processors can ever contend 
        for names in $G_{j''>j}$, therefore, $\alpha n$ safe iterations can occur only if in 
        at most $\frac{n}{2^{j}}$ of them processors choose to contend in $G_{j''>j}$.
Otherwise, some processor would have to complete an iteration where it contended 
        for a name in $G_{j''>j}$.
        
In every $\id{clean}(j)$ iteration, at line~\ref{line:pickspot}, 
        any processor $p$ contends for a name in $G_{j' \geq j}$ uniformly at random 
        among non-contended spots in its view $V_p$.
With probability at least $\frac{1}{2}$, $p$ contends for a name from $G_{j''>j}$,
        because by definition of $\id{clean}(j)$, 
        all spots in $G_{j''>j}$ are non-contended in $V_p$.

Let us describe the process by considering a random variable 
        $Z \sim \mathrm{B}(\alpha n, \frac{1}{2})$ for $\alpha \geq \frac{1}{2^{j-5}}$,
        where each success event corresponds to an iteration contending in $G_{j''>j}$.
By the Chernoff Bound, the probability of $\alpha n$ iterations with at most
        $\frac{n}{2^{j}}$ processors contending in $G_{j''>j}$ is:
\begin{align*}
\Pr\left[Z \leq \frac{n}{2^j}\right] = 
\Pr\left[Z \leq \frac{\alpha n}{2} \left( 1 - \frac{2^{j-1} \alpha - 1}{2^{j-1} \alpha}\right)\right]
\leq \exp\left(- \frac{\alpha n (2^{j-1} \alpha - 1)^2}{2 (2^{j-1} \alpha)^2} \right)
\leq e^{-\frac{\alpha n}{8}}
\end{align*}
So far, we have assumed that the set of names belonging to the later groups $G_{j''>j}$ was fixed,
        but the the adversary controls the execution.
Luckily, what happened before phase $j$ (i.e. the actual names that were acquired from $G_{j'''<j}$)
        is irrelevant, because all the names from the earlier phases
        are viewed as contended by all iterations that start in phases $j' \geq j$.
Unfortunately, however, the adversary also influences what names belong to
        group $j$ and to groups $G_{j''>j}$.
There are $\binom{2^{1-j}n}{2^{-j}n}$ different possible choices for names in $G_j$, 
        and by a union bound, the probability that $\alpha n$ iterations can occur 
        even for one of them is at most:
\begin{align*}
e^{-\frac{\alpha n}{8}} \cdot \binom{2^{1-j}n}{2^{-j}n}
\leq e^{-\frac{\alpha n}{8}} \cdot (2e)^{2^{-j}n}
\leq e^{-n (2^{-3}\alpha - 2^{1-j})}
\leq e^{-\frac{\alpha n}{16}}
\end{align*}
\noindent proving the claim.
\end{proof}
\noindent Plugging $\alpha = \beta - \frac{1}{2^{j-1}} \geq \frac{1}{2^{j-5}}$ in the above lemma,
        we obtain the following
\begin{corollary}
\label{cor:expdec}
The total number of $\id{clean}(j)$ iterations 
        is larger than or equal to $\beta n$ with probability 
        at most $e^{-\frac{\beta n}{32}}$ for all $\beta \geq \frac{1}{2^{j-6}}$.
\end{corollary}
%\begin{proof}
%  Let us plug $\alpha = \beta - \frac{1}{2^{j-1}} \geq \frac{1}{2^{j-5}}$
%        into~\lemmaref{lem:phaseunion}.
%Then, the probability of experiencing at least $\beta n$ $\id{clean}(j)$ iterations is
%        at most $e^{-\frac{\alpha n}{16}} \leq e^{-\frac{\beta n}{32}}$.
%\end{proof}
\noindent Let $X_i(\id{clean})$ be the number of processors that ever contend for 
        $u_i \in G_j$ in some $\id{clean}(j)$ iteration and define $X_i(\id{dirty})$ analogously:
        as the number of processors that ever contend for 
        $u_i \in G_j$ in some $\id{dirty}(j)$ iteration.
Relying on~\corollaryref{cor:expdec}, we get the following result:
\begin{replemma}{lem:rentype1}
$\mathbb{E}[\sum_{i=1}^n X_i(\id{clean})] = O(n).$
\end{replemma}
\noindent Complete proofs of the above and following lemmas
        can be found in~\appendixref{app:tasproofs}.
Each iteration where a processor contends for a name $u_i \in G_j$ is by definition
        either as $\id{clean}(j)$, $\id{dirty}(j)$ or starts in a phase $j''' < j$.
Let us call these $\id{cross}(j)$  and denote by $X_i(\id{cross})$ the number of such iterations.
\begin{replemma}{lem:notwice}
  In any execution, for each $j$, any processor participates in at most one $\id{dirty}(j)$
        and at most one $\id{cross}(j)$ iteration.
\end{replemma}
\begin{replemma}{lem:rentype23}
$\mathbb{E}[\sum_{i=1}^n X_i(\id{dirty})] = O(n)$ and 
        $\mathbb{E}[\sum_{i=1}^n X_i(\id{cross})] = O(n).$
\end{replemma}
\noindent The message complexity upper bound then follows by piecing together the previous claims. 
\begin{theorem}
The expected message complexity of our renaming algorithm is $O(n^2)$.
\end{theorem}
\begin{proof}
We know $X_i = X_i(\id{clean}) + X_i(\id{dirty}) + X_i(\id{cross})$ 
        and by~\lemmaref{lem:rentype1},~\lemmaref{lem:rentype23}
        we get $\mathbb{E}[\sum_i X_i] = O(n)$.
Combining with~\lemmaref{lem:msgrenameweak} gives the desired result.
\end{proof}
\noindent The round complexity upper bound exploits a  
 trade-off between the probability 
that a processor collides in an iteration (and must continue) and 
the ratio of available slots which must become assigned during that iteration. 
\begin{reptheorem}{thm:rounds}
The round complexity of the renaming protocol is $O( \log^2 n )$, with high probability. 
\end{reptheorem}
\begin{proof}[Proof Sketch]
We fix an arbitrary processor $p$, and upper bound the number of loop iterations it performs during the execution. 
Let $M_i$ be the set of free slots that $p$ sees when performing its random choice in the $i$th iteration of the loop, 
and let $m_i = |M_i|$. 

Assuming that $p$ does not complete in iteration $i$, let $Y_i \subseteq M_i$ be the set of \emph{new} slots that $p$ finds out have become contended at the beginning of iteration $i + 1$, and let $y_i = |Y_i|$. 
We define an iteration as \emph{low-information} if $y_i / m_i < 1 / \log m_i$.  
Intuitively, in a high-information iteration, the processor collides, but at least reduces its random range for choices by a significant factor.  

We then focus on a low-information iteration $i$. 
We model the interaction between the processor and the adversary as follows: 
$p$ first makes a random choice among $m_i$ slots. The adversary can then schedule 
$m_i - 1$ other processors to make choices in $M_i$. 
Importantly, we note that the adversary can schedule some processors several times; however, for each such re-scheduling, it must announce the previously chosen slot. 
A balls-into-bins argument yields that the adversary can obtain at most $m_i$  
extra choices for the iteration to stay \emph{low-information}, with probability at least $1 - 1 / m_i$. 

Recall that the goal of the adversary is to cause a collision with $p$'s random choice $r$. 
We reduce this to a balls-into-bins game in which the adversary throws at most $2m_i - 1$ initial balls  
into a set of $m_i ( 1 - 1 / \log m_i)$ bins, with the goal of hitting a specific bin, corresponding to $p$'s random choice. 
However, the probability that an arbitrary bin gets hit in this game is at most a constant. 

By the above, processor $p$ terminates in each low-information iteration with constant probability. 
Putting it all together, we obtain that, for $c \geq 4$ constant, after $c \log^2 n$ iterations, any processor $p$ will terminate with probability $1 - 1 / n^{c - 1}$, 
either because $m_i$ reaches $1$, or because one of its probes was successful in an low-information phase, which occurs with high probability. 
\end{proof}

